Session Types at the Mirror

We (re)define session types as projections of process behaviors with respect to the communication channels they use. In this setting, we give session types a semantics based on fair testing. The outcome is a unified theory of behavioral types that shares common aspects with conversation types and that encompass features of both dyadic and multi-party session types. The point of view we provide sheds light on the nature of session types and gives us a chance to reason about them in a framework where every notion, from well-typedness to the subtyping relation between session types, is semantically -rather than syntactically- grounded.

==> eptcsdata.tex <==
\providecommand{\event}{F. Bonchi, D. Grohmann, P. Spoletini, and E. Tuosto:\\ 
   ICE'09 Structured Interactions}
\providecommand{\volume}{12}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{71}
\providecommand{\eid}{5}

